Hyperledger Fabric Blockchain and ROS 2 Integration for Autonomous Mobile Robots

In industrial applications, security and trust in the system are requirements for widespread adoption. Blockchain technologies have emerged as a potential solution to address identity management and secure data aggregation and control. However, the vast majority of works to date utilize Ethereum and smart contracts that are not scalable or well suited for industrial applications. This paper presents what is, to the best of our knowledge, the first integration of ROS 2 with the Hyperledger Fabric blockchain. With a framework that leverages Fabric smart contracts and ROS 2 through a Go application, we delve into the potential of using blockchain for controlling robots, and gathering and processing their data. We demonstrate the applicability of the proposed framework to an inventory management use-case where different robots are used to detect objects of interest in a given area. Designed to meet the requirements of distributed robotic systems, we show that the performance of the robots is not impacted significantly by the blockchain layer. At the same time, we provide examples for developing other applications that integrate Fabric smart contracts with ROS 2. Our results pave the way for further adoption of blockchain technologies in autonomous robotic systems for building trustable data sharing.

==> algs/general.tex <==
\begin{algorithm}[t]
    \normalsize
	\caption{ROS2 + Hyperledger Fabric Application}
	\label{alg:localization_algotirhm}
	\KwIn{\\
	    \hspace{1em} Localizations; \\
	    \hspace{1em} Detected Object; \\
	}
	\KwOut{\\
	    \hspace{1em} Assets in the smart contract;
	}  
	\BlankLine
% 	Calculate $L(\mathcal{G})$;\\
    \While {Network is Up} {
        \If{Chaincode1 deployed to the channel} {
            Smart contracts are accessible to an App;\\
            \While {Tello1 Follows Path1} {
                Ros2 node1 publish a position;\\
                \ForEach{published position} {
                   Ros2 node1 in the App subscribes to the $\setminus$position topic;\\
                   Positions are stored in a smart contract1;\\
                } 
                \If{Tello1 detects an object} {
                    Ros2 node2 publish a photo of the object;\\
                    \ForEach{published photo} {
                        Ros2 node2 in the App subscribes to the $\setminus$object-detection topic;\\
                        The object type with it's position are stored in smart contract2;\\
                    } 
                }
            }
        }
        \If{Chaincode2 deployed to the channel} {
            Smart contracts are accessible to an App;\\
            \While {Tello2 Follows Path2} {
                Ros2 node1 publish a position;\\
                \ForEach{published position} {
                        Ros2 node1 in the App subscribes to the $\setminus$position topic;\\
                        Positions are stored in a smart contract1;\\
                    } 
                \If{Tello2 detects an object} {
                    Ros2 node2 publish a photo of the object;\\
                    \ForEach{published photo} {
                        Ros2 node2 in the App subscribes to the $\setminus$object-detection topic;\\
                        The object type with it's position are stored in smart contract2;\\
                    } 
                }
            }
        }
    }
\end{algorithm}

==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}

==> sec/06_Experiments_BACKUP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%%              EXPERIMENTS                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Experimental Results}

We demonstrated the usability of the proposed framework with a proof of concept, where multiple robots, ground and aerial robot, are used for object detection in the determined area. Hyperledger Fabric is used as a communication tool for storing data and controlling robots through a Go application and integration of smart contracts with ROS2. 



\subsection{Experimental setup}

\textbf{Heterogeneous Multi-Robot System.} The employed multi-robot system in this paper, consists of a ground robot and a unmanned aerial vehicle (UAV). The ground robot is an EAI Dashgo platform equipped with a Livox Horizon lidar. 
The custom-built UAV is based on the X500 quad-rotor frame which is embedded with a Pixhawk flight controller running the PX4 firmware. A TF Mini Lidar is utilized for height estimation on the UAV, also equipped with Intel RealSense D435 depth camera for sensing and 3D reconstruction. An AAEON Up Square with dual-code Intel Celeron processor is used as a companion computer on both robots. Both robots use RealSense T265 cameras for VIO-based egomotion estimation.

\red{
\textbf{UWB Ranging and Position Estimation.} The distance between each pair of robots is estimated using Decawave DWM1001 UWB transceivers. In order to ensure a safe fallback for the MAV autonomous flight, we utilize both an anchor-based localization system as well as ranging between robots for collaborative localization.}



\subsection{Deployment of the ROS~2 Fabric Network and Application}

After bringing up the network, consists of two organizations, two peer nodes and one ordering node, Fabric channel is created for transactions between organizations which are a private layer of communication between specific network members. Channels can be used only by organizations that are invited to the channel, and are invisible to other members of the network. Organizations that have been invited, join their peers to the channel to store the channel ledger and validate the transactions on the channel.

After creating the channel, smart contracts can be used to interact with the channel ledger. A Chaincode is installed on the peers of an organization and then deployed to a channel, where it can then be used to endorse transactions and interact with the blockchain ledger. 

After invoking the chaincode, application can be used to interact with a blockchain network by submitting transactions to a ledger or querying ledger content. Applications run by members of the network can invoke smart contracts to create assets on the ledger, as well as change and transfer those assets. Applications also query smart contracts to read data on the ledger.

\subsection{Fabric channels and smart contracts}

For the implementation of the different parts of the system, the Go programming language (golang), for the smart contracts and applications are used. Also the private network (Hyperledger Fabric) has been brought up for secure data management and robot control, which consists of various process as follows.
\begin{enumerate}
  \item create one orderer and two organizations, Org1 and Org2, consists of one peer each
  \item generate genesis block and bring up docker containers after creating certificates for organizations
  \item Create channel genesis block and then join the peers of organizations to the channel and set anchor peers for each in the channel
  \item approving the definition of the chaincode for organizations after packaging and installing them on peers
  \item Invoking the chincode after commitment of definitions successfully 
\end{enumerate}

Two smart contracts, one for storing the path location of the robots and one for storing the location of the detected objects in the asset have been used in this implementation. For each robot one application has been used which has various functions for controlling the assets, such as creating new assets, read all the assets, check existence of the assets, updating the assets and also changing them.

\red{\textbf{Software.} Robots are running ROS Melodic under Ubuntu 18.04. Localization and object detection are running ROS2 foxy under ubuntu 20.04. Smart contracts, applications and most of the codes are written in Go programming language (golang), and  all the code utilized in this paper is open-source and will be made freely available in our GitHub page\footnote{\url{https://github.com/TIERS}}.}

\begin{figure*}
    \centering
    \includegraphics[width=.95\textwidth]{fig/IROS_implementation_thin.pdf}
    \caption{{Implementation Diagram}}
    \label{fig:implementation}
\end{figure*}



\subsection{Results}

- Trajectory, points that have been stored in the chaincode (drone location + object locations)

- CPU + RAM usage

- Latency of the fabric transactions



\begin{figure}
    \centering
    \setlength\figureheight{0.23\textwidth}
    \setlength\figurewidth{0.49\textwidth}
    \scriptsize{\input{algs/graphs/trajectory}}
    \caption{Trajectory Tracking}
    \label{fig:drone_trajectory}
\end{figure}
\begin{figure}
    \centering
    \setlength\figureheight{0.23\textwidth}
    \setlength\figurewidth{0.49\textwidth}
    \scriptsize{\input{algs/graphs/ram_plot}}
    \caption{Memory Usage}
    \label{fig:error_distance_node5}
\end{figure}
\begin{figure}
    \centering
    \setlength\figureheight{0.23\textwidth}
    \setlength\figurewidth{0.49\textwidth}
    \scriptsize{\input{algs/graphs/CPU_plot}}
    \caption{CPU Usage}
    \label{fig:error_distance_node5}
\end{figure}

\begin{table*}
\begin{tabularx}{\textwidth}{@{}l*{12}{c}c@{}}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Batch \\ Timeout(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max \\ Messages\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max \\ Frequency(Hz)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Delay\\ (Miliseconds)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Average\\  CPU(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Average \\ Memory(MB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Orderer \\ CPU(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Orderer \\ Mem(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Peer Org1\\  CPU(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Peer Org1\\  Mem(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Peer Org2 \\ CPU(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Peer Org2 \\ Mem(\%)\end{tabular} \\ \hline
5                                                           & 5                                                       & 182.7                                                        & 5                                                             & 90                                                         & 50                                                            & 28.1                                                       & \begin{tabular}[c]{@{}c@{}}9\%\\ 57.51MiB\end{tabular}     & 68.49                                                        & \begin{tabular}[c]{@{}c@{}}12\%\\ 75.82MiB\end{tabular}      & 63.4                                                         & \begin{tabular}[c]{@{}c@{}}12\%\\ 75.2MiB\end{tabular}       \\ \hline
5                                                           & 10                                                      & 118                                                          & 5                                                             & 90                                                         & 49                                                            & 30                                                         & \begin{tabular}[c]{@{}c@{}}13\%\\ 84.23MiB\end{tabular}    & 73.73                                                        & \begin{tabular}[c]{@{}c@{}}14\%\\ 86.69MiB\end{tabular}      & 70.39                                                        & \begin{tabular}[c]{@{}c@{}}14\%\\ 88.41MiB\end{tabular}      \\ \hline
5                                                           & 20                                                      & 69                                                           & 5                                                             & 90                                                         & 48.5                                                          & 23.67                                                      & \begin{tabular}[c]{@{}c@{}}8\%\\ 53.95MiB\end{tabular}     & 74                                                           & \begin{tabular}[c]{@{}c@{}}13\%\\ 83.63MiB\end{tabular}      & 70                                                           & \begin{tabular}[c]{@{}c@{}}14\%\\ 90.92MiB\end{tabular}      \\ \hline
5                                                           & 40                                                      & 40.5                                                         & 5                                                             & 90                                                         & 49                                                            & 22.9                                                       & \begin{tabular}[c]{@{}c@{}}9\%\\ 60.73MiB\end{tabular}     & 72.56                                                        & \begin{tabular}[c]{@{}c@{}}15\%\\ 96.45MiB\end{tabular}      & 73.75                                                        & \begin{tabular}[c]{@{}c@{}}14\%\\ 88.94MiB\end{tabular}      \\ \hline
5                                                           & 50                                                      & 36                                                           & 5                                                             & 89                                                         & 48                                                            & 19.55                                                      & \begin{tabular}[c]{@{}c@{}}11\%\\ 72.46MiB\end{tabular}    & 72.62                                                        & \begin{tabular}[c]{@{}c@{}}16\%\\ 105MiB\end{tabular}        & 72.85                                                        & \begin{tabular}[c]{@{}c@{}}16\%\\ 104.9MiB\end{tabular}      \\ \hline
5                                                           & 100                                                     & 28.5                                                         & 5                                                             & 85                                                         & 46                                                            & 24.98                                                      & \begin{tabular}[c]{@{}c@{}}9\%\\ 57.44MiB\end{tabular}     & 71.91                                                        & \begin{tabular}[c]{@{}c@{}}16\%\\ 104.7MiB\end{tabular}      & 70.98                                                        & \begin{tabular}[c]{@{}c@{}}18\%\\ 113.3MiB\end{tabular}      \\ \hline
5                                                           & 200                                                     & 29                                                           & 5                                                             & 88                                                         & 49                                                            & 22.97                                                      & \begin{tabular}[c]{@{}c@{}}10\%\\ 62.99MiB\end{tabular}    & 72.81                                                        & \begin{tabular}[c]{@{}c@{}}18\%\\ 117.9MiB\end{tabular}      & 73.26                                                        & \begin{tabular}[c]{@{}c@{}}19\%\\ 119.8MiB\end{tabular}      \\ \hline
5                                                           & 500                                                     & 29                                                           & 5                                                             & 88                                                         & 49                                                            & 22.64                                                      & \begin{tabular}[c]{@{}c@{}}11\%\\ 69.86MiB\end{tabular}    & 70.98                                                        & \begin{tabular}[c]{@{}c@{}}17\%\\ 11.9MiB\end{tabular}       & 71.67                                                        & \begin{tabular}[c]{@{}c@{}}18\%\\ 112.9MiB\end{tabular}      \\ \hline
5                                                           & 1000                                                    & 27                                                           & 5                                                             & 89                                                         & 49                                                            & 23                                                         & \begin{tabular}[c]{@{}c@{}}10 \% \\ 61.57 MiB\end{tabular} & 75                                                           & \begin{tabular}[c]{@{}c@{}}18\%\\ 116.6MiB\end{tabular}      & 75                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 106.8MiB\end{tabular}      \\ \hline
5                                                           & 2000                                                    & 30.5                                                         & 5                                                             & 89                                                         & 49                                                            & 23                                                         & \begin{tabular}[c]{@{}c@{}}0.11\%\\ 70MiB\end{tabular}     & 73                                                           & \begin{tabular}[c]{@{}c@{}}19\%\\ 119.1MiB\end{tabular}      & 73                                                           & \begin{tabular}[c]{@{}c@{}}19\%\\ 121.7MiB\end{tabular}      \\ \hline
5                                                           & 3000                                                    & 27                                                           & 5                                                             & 88                                                         & 50                                                            & 20                                                         & \begin{tabular}[c]{@{}c@{}}9\%\\ 56.41MiB\end{tabular}     & 74                                                           & \begin{tabular}[c]{@{}c@{}}16\%\\ 104.2MiB\end{tabular}      & 73                                                           & \begin{tabular}[c]{@{}c@{}}16\%\\ 105.2MiB\end{tabular}      \\ \hline
0.1                                                         & 100                                                     & 70                                                           & 5                                                             & 90                                                         & 49                                                            & 20.71                                                      & \begin{tabular}[c]{@{}c@{}}8\%\\ 51.88MiB\end{tabular}     & 70                                                           & \begin{tabular}[c]{@{}c@{}}13\%\\ 83MiB\end{tabular}         & 71                                                           & \begin{tabular}[c]{@{}c@{}}13\%\\ 83MiB\end{tabular}         \\ \hline
0.5                                                         & 100                                                     & 26                                                           & 5                                                             & 89                                                         & 49                                                            & 26.7                                                       & \begin{tabular}[c]{@{}c@{}}11\%\\ 70.75MiB\end{tabular}    & 73                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 109MiB\end{tabular}        & 72                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 109MiB\end{tabular}        \\ \hline
1                                                           & 100                                                     & 25.5                                                         & 5                                                             & 89                                                         & 49                                                            & 22.82                                                      & \begin{tabular}[c]{@{}c@{}}13\%\\ 80.65MiB\end{tabular}    & 73                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 108MiB\end{tabular}        & 74                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 108.7MiB\end{tabular}      \\ \hline
2                                                           & 100                                                     & 24                                                           & 5                                                             & 89                                                         & 49                                                            & 27                                                         & \begin{tabular}[c]{@{}c@{}}10\%\\ 66.76MiB\end{tabular}    & 72                                                           & \begin{tabular}[c]{@{}c@{}}18\%\\ 117.7MiB\end{tabular}      & 70                                                           & \begin{tabular}[c]{@{}c@{}}17\%\\ 106.8MiB\end{tabular}      \\ \hline
0.09                                                        & 100                                                     & 73.5                                                         & 5                                                             & 90                                                         & 47                                                            & 28                                                         & \begin{tabular}[c]{@{}c@{}}10\%\\ 62.94MiB\end{tabular}    & 71                                                           & \begin{tabular}[c]{@{}c@{}}14\%\\ 92MiB\end{tabular}         & 70                                                           & \begin{tabular}[c]{@{}c@{}}13\%\\ 85.64MiB\end{tabular}      \\ \hline
0.06                                                        & 100                                                     & 103                                                          & 5                                                             & 91                                                         & 49                                                            & 29                                                         & \begin{tabular}[c]{@{}c@{}}9\%\\ 60.44MiB\end{tabular}     & 71                                                           & \begin{tabular}[c]{@{}c@{}}13\%\\ 84.55MiB\end{tabular}      & 71                                                           & \begin{tabular}[c]{@{}c@{}}14\%\\ 89.09MiB\end{tabular}      \\ \hline
0.05                                                        & 100                                                     & 114                                                          & 5                                                             & 91                                                         & 48                                                            & 26                                                         & \begin{tabular}[c]{@{}c@{}}9\%\\ 55.8MiB\end{tabular}      & 69.5                                                         & \begin{tabular}[c]{@{}c@{}}14\%\\ 89MiB\end{tabular}         & 69.42                                                        & \begin{tabular}[c]{@{}c@{}}12\%\\ 77.42MiB\end{tabular}      \\ \hline
0.01                                                        & 100                                                     & 128                                                          & 5                                                             & 82                                                         & ?                                                             & 29                                                         & \begin{tabular}[c]{@{}c@{}}16\%\\ 101MiB\end{tabular}      & 58                                                           & \begin{tabular}[c]{@{}c@{}}16\%\\ 103MiB\end{tabular}        & 56                                                           & \begin{tabular}[c]{@{}c@{}}15\%\\ 96.2Mib\end{tabular}       \\ \hline
0.025                                                       & 100                                                     & 155                                                          & 5                                                             & 92                                                         & 48                                                            & 28                                                         & \begin{tabular}[c]{@{}c@{}}10\%\\ 61.89MiB\end{tabular}    & 71                                                           & \begin{tabular}[c]{@{}c@{}}10\%\\ 85MiB\end{tabular}         & 71                                                           & \begin{tabular}[c]{@{}c@{}}12\%\\ 74MiB\end{tabular}         \\ \hline
\end{tabular}
\end{tabularx}
\end{table*}


==> tex/square_boxplot_navi_xy.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.91796875,0.25,0.203125}
\definecolor{color1}{rgb}{0.6328125,0.203125,0.91796875}
\definecolor{color2}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color3}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color4}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color5}{rgb}{0.854901960784314,0.647058823529412,0.125490196078431}
\definecolor{color6}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
\definecolor{color7}{rgb}{0.627450980392157,0.32156862745098,0.176470588235294}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    tick align=outside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    xtick style={color=black},
    y grid style={white!90!black},
    ymajorgrids,
    ytick style={color=black},
    scaled y ticks = false,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=0.666,
      text opacity=1,
      at={(0.97,0.97)},
      anchor=north east,
      draw=white!80!black
    },
    tick align=outside,
    tick pos=left,
    %
    %
    %
    %
    %
    %
    %
    log basis y={10},
    % tick align=outside,
    % tick pos=left,
    % title={XY Navigation Errors Based on Different Anchor Distribution at Heights of 5, 10 and 20 meters},
    % x grid style={white!69.0196078431373!black},
    xmin=-0.5, xmax=26,
    % xtick style={color=black},
    xtick={3.5,13,23},
    xticklabels={5m,10m,20m},
    % y grid style={white!69.0196078431373!black},
    ymin=0.00823407310056917, ymax=2.7,
    ymode=log,
    % ytick style={color=black}
]
\addplot [line width=1pt, color0, forget plot]
table {%
-0.25 0.0629254579544067
0.25 0.0629254579544067
0.25 0.116854261331483
0.125 0.133378744125366
0.25 0.149903226919249
0.25 0.225299537181854
-0.25 0.225299537181854
-0.25 0.149903226919249
-0.125 0.133378744125366
-0.25 0.116854261331483
-0.25 0.0629254579544067
};
\addplot [black, forget plot]
table {%
0 0.0629254579544067
0 0.0100212097167969
};
\addplot [black, forget plot]
table {%
0 0.225299537181854
0 0.464566707611084
};
\addplot [black, forget plot]
table {%
-0.125 0.0100212097167969
0.125 0.0100212097167969
};
\addplot [black, forget plot]
table {%
-0.125 0.464566707611084
0.125 0.464566707611084
};
\addplot [line width=1pt, color2, forget plot]
table {%
0.75 0.0550479888916016
1.25 0.0550479888916016
1.25 0.0872549469128582
1.125 0.0913627147674561
1.25 0.0954704826220539
1.25 0.136493682861328
0.75 0.136493682861328
0.75 0.0954704826220539
0.875 0.0913627147674561
0.75 0.0872549469128582
0.75 0.0550479888916016
};
\addplot [black, forget plot]
table {%
1 0.0550479888916016
1 0.0105924606323242
};
\addplot [black, forget plot]
table {%
1 0.136493682861328
1 0.256451845169067
};
\addplot [black, forget plot]
table {%
0.875 0.0105924606323242
1.125 0.0105924606323242
};
\addplot [black, forget plot]
table {%
0.875 0.256451845169067
1.125 0.256451845169067
};
\addplot [line width=1pt, color3, forget plot]
table {%
1.75 0.0262908935546875
2.25 0.0262908935546875
2.25 0.0422004902930734
2.125 0.0437288284301758
2.25 0.0452571665672782
2.25 0.0594601631164551
1.75 0.0594601631164551
1.75 0.0452571665672782
1.875 0.0437288284301758
1.75 0.0422004902930734
1.75 0.0262908935546875
};
\addplot [black, forget plot]
table {%
2 0.0262908935546875
2 0.010059118270874
};
\addplot [black, forget plot]
table {%
2 0.0594601631164551
2 0.108749151229858
};
\addplot [black, forget plot]
table {%
1.875 0.010059118270874
2.125 0.010059118270874
};
\addplot [black, forget plot]
table {%
1.875 0.108749151229858
2.125 0.108749151229858
};
\addplot [line width=1pt, color4, forget plot]
table {%
2.75 0.111529111862183
3.25 0.111529111862183
3.25 0.130515317329696
3.125 0.196047306060791
3.25 0.261579294791886
3.25 0.24996542930603
2.75 0.24996542930603
2.75 0.261579294791886
2.875 0.196047306060791
2.75 0.130515317329696
2.75 0.111529111862183
};
\addplot [black, forget plot]
table {%
3 0.111529111862183
3 0.0505809783935547
};
\addplot [black, forget plot]
table {%
3 0.24996542930603
3 0.389389276504517
};
\addplot [black, forget plot]
table {%
2.875 0.0505809783935547
3.125 0.0505809783935547
};
\addplot [black, forget plot]
table {%
2.875 0.389389276504517
3.125 0.389389276504517
};
\addplot [line width=1pt, color5, forget plot]
table {%
3.75 0.0398937463760376
4.25 0.0398937463760376
4.25 0.0386781307707235
4.125 0.0503287315368652
4.25 0.061979332303007
4.25 0.150957584381104
3.75 0.150957584381104
3.75 0.061979332303007
3.875 0.0503287315368652
3.75 0.0386781307707235
3.75 0.0398937463760376
};
\addplot [black, forget plot]
table {%
4 0.0398937463760376
4 0.0105338096618652
};
\addplot [black, forget plot]
table {%
4 0.150957584381104
4 0.312473297119141
};
\addplot [black, forget plot]
table {%
3.875 0.0105338096618652
4.125 0.0105338096618652
};
\addplot [black, forget plot]
table {%
3.875 0.312473297119141
4.125 0.312473297119141
};
\addplot [line width=1pt, color6, forget plot]
table {%
4.75 0.0273342132568359
5.25 0.0273342132568359
5.25 0.0339629243246975
5.125 0.0363602638244629
5.25 0.0387576033242283
5.25 0.0742993354797363
4.75 0.0742993354797363
4.75 0.0387576033242283
4.875 0.0363602638244629
4.75 0.0339629243246975
4.75 0.0273342132568359
};
\addplot [black, forget plot]
table {%
5 0.0273342132568359
5 0.010307788848877
};
\addplot [black, forget plot]
table {%
5 0.0742993354797363
5 0.141448497772217
};
\addplot [black, forget plot]
table {%
4.875 0.010307788848877
5.125 0.010307788848877
};
\addplot [black, forget plot]
table {%
4.875 0.141448497772217
5.125 0.141448497772217
};
\addplot [line width=1pt, color0, forget plot]
table {%
9.75 0.109080791473389
10.25 0.109080791473389
10.25 0.208775860281895
10.125 0.217644453048706
10.25 0.226513045815517
10.25 0.355952739715576
9.75 0.355952739715576
9.75 0.226513045815517
9.875 0.217644453048706
9.75 0.208775860281895
9.75 0.109080791473389
};
\addplot [black, forget plot]
table {%
10 0.109080791473389
10 0.0106794834136963
};
\addplot [black, forget plot]
table {%
10 0.355952739715576
10 0.499023914337158
};
\addplot [black, forget plot]
table {%
9.875 0.0106794834136963
10.125 0.0106794834136963
};
\addplot [black, forget plot]
table {%
9.875 0.499023914337158
10.125 0.499023914337158
};
\addplot [line width=1pt, color2, forget plot]
table {%
10.75 0.061793327331543
11.25 0.061793327331543
11.25 0.119313400273
11.125 0.124480247497559
11.25 0.129647094722117
11.25 0.237082719802856
10.75 0.237082719802856
10.75 0.129647094722117
10.875 0.124480247497559
10.75 0.119313400273
10.75 0.061793327331543
};
\addplot [black, forget plot]
table {%
11 0.061793327331543
11 0.0100317001342773
};
\addplot [black, forget plot]
table {%
11 0.237082719802856
11 0.498574733734131
};
\addplot [black, forget plot]
table {%
10.875 0.0100317001342773
11.125 0.0100317001342773
};
\addplot [black, forget plot]
table {%
10.875 0.498574733734131
11.125 0.498574733734131
};
\addplot [line width=1pt, color3, forget plot]
table {%
11.75 0.0356164574623108
12.25 0.0356164574623108
12.25 0.0590718957655501
12.125 0.0608000755310059
12.25 0.0625282552964616
12.25 0.0943392515182495
11.75 0.0943392515182495
11.75 0.0625282552964616
11.875 0.0608000755310059
11.75 0.0590718957655501
11.75 0.0356164574623108
};
\addplot [black, forget plot]
table {%
12 0.0356164574623108
12 0.0100545883178711
};
\addplot [black, forget plot]
table {%
12 0.0943392515182495
12 0.180632591247559
};
\addplot [black, forget plot]
table {%
11.875 0.0100545883178711
12.125 0.0100545883178711
};
\addplot [black, forget plot]
table {%
11.875 0.180632591247559
12.125 0.180632591247559
};
\addplot [line width=1pt, color4, forget plot]
table {%
12.75 0.0324709415435791
13.25 0.0324709415435791
13.25 0.0561843826720145
13.125 0.0580892562866211
13.25 0.0599941299012277
13.25 0.0934865474700928
12.75 0.0934865474700928
12.75 0.0599941299012277
12.875 0.0580892562866211
12.75 0.0561843826720145
12.75 0.0324709415435791
};
\addplot [black, forget plot]
table {%
13 0.0324709415435791
13 0.0100338459014893
};
\addplot [black, forget plot]
table {%
13 0.0934865474700928
13 0.184965848922729
};
\addplot [black, forget plot]
table {%
12.875 0.0100338459014893
13.125 0.0100338459014893
};
\addplot [black, forget plot]
table {%
12.875 0.184965848922729
13.125 0.184965848922729
};
\addplot [line width=1pt, color5, forget plot]
table {%
13.75 0.0223686695098877
14.25 0.0223686695098877
14.25 0.035463001367267
14.125 0.0366926193237305
14.25 0.0379222372801939
14.25 0.062411367893219
13.75 0.062411367893219
13.75 0.0379222372801939
13.875 0.0366926193237305
13.75 0.035463001367267
13.75 0.0223686695098877
};
\addplot [black, forget plot]
table {%
14 0.0223686695098877
14 0.0100116729736328
};
\addplot [black, forget plot]
table {%
14 0.062411367893219
14 0.121386528015137
};
\addplot [black, forget plot]
table {%
13.875 0.0100116729736328
14.125 0.0100116729736328
};
\addplot [black, forget plot]
table {%
13.875 0.121386528015137
14.125 0.121386528015137
};
\addplot [line width=1pt, color6, forget plot]
table {%
14.75 0.0270559787750244
15.25 0.0270559787750244
15.25 0.0513307469276914
15.125 0.053499698638916
15.25 0.0556686503501407
15.25 0.0965852737426758
14.75 0.0965852737426758
14.75 0.0556686503501407
14.875 0.053499698638916
14.75 0.0513307469276914
14.75 0.0270559787750244
};
\addplot [black, forget plot]
table {%
15 0.0270559787750244
15 0.0100679397583008
};
\addplot [black, forget plot]
table {%
15 0.0965852737426758
15 0.198929309844971
};
\addplot [black, forget plot]
table {%
14.875 0.0100679397583008
15.125 0.0100679397583008
};
\addplot [black, forget plot]
table {%
14.875 0.198929309844971
15.125 0.198929309844971
};
\addplot [line width=1pt, color0]
table {%
19.75 0.133109569549561
20.25 0.133109569549561
20.25 0.251491091482432
20.125 0.263442993164062
20.25 0.275394894845693
20.25 0.394724369049072
19.75 0.394724369049072
19.75 0.275394894845693
19.875 0.263442993164062
19.75 0.251491091482432
19.75 0.133109569549561
};
%\addlegendentry{0.6 * 0.6}
\addplot [black, forget plot]
table {%
20 0.133109569549561
20 0.0112812519073486
};
\addplot [black, forget plot]
table {%
20 0.394724369049072
20 0.498894691467285
};
\addplot [black, forget plot]
table {%
19.875 0.0112812519073486
20.125 0.0112812519073486
};
\addplot [black, forget plot]
table {%
19.875 0.498894691467285
20.125 0.498894691467285
};
\addplot [line width=1pt, color2]
table {%
20.75 0.112098932266235
21.25 0.112098932266235
21.25 0.204240932496009
21.125 0.21213698387146
21.25 0.220033035246911
21.25 0.353559255599976
20.75 0.353559255599976
20.75 0.220033035246911
20.875 0.21213698387146
20.75 0.204240932496009
20.75 0.112098932266235
};
%\addlegendentry{1.2 * 1.2}
\addplot [black, forget plot]
table {%
21 0.112098932266235
21 0.010089635848999
};
\addplot [black, forget plot]
table {%
21 0.353559255599976
21 0.499281406402588
};
\addplot [black, forget plot]
table {%
20.875 0.010089635848999
21.125 0.010089635848999
};
\addplot [black, forget plot]
table {%
20.875 0.499281406402588
21.125 0.499281406402588
};
\addplot [line width=1pt, color3]
table {%
21.75 0.0613045692443848
22.25 0.0613045692443848
22.25 0.107318790443975
22.125 0.11083984375
22.25 0.114360897056025
22.25 0.179744243621826
21.75 0.179744243621826
21.75 0.114360897056025
21.875 0.11083984375
21.75 0.107318790443975
21.75 0.0613045692443848
};
%\addlegendentry{3.0 * 3.0}
\addplot [black, forget plot]
table {%
22 0.0613045692443848
22 0.0102958679199219
};
\addplot [black, forget plot]
table {%
22 0.179744243621826
22 0.353663444519043
};
\addplot [black, forget plot]
table {%
21.875 0.0102958679199219
22.125 0.0102958679199219
};
\addplot [black, forget plot]
table {%
21.875 0.353663444519043
22.125 0.353663444519043
};
\addplot [line width=1pt, color4]
table {%
22.75 0.0401172637939453
23.25 0.0401172637939453
23.25 0.0776253280932044
23.125 0.0806457996368408
23.25 0.0836662711804773
23.25 0.13330078125
22.75 0.13330078125
22.75 0.0836662711804773
22.875 0.0806457996368408
22.75 0.0776253280932044
22.75 0.0401172637939453
};
%\addlegendentry{4.0 * 4.0}
\addplot [black, forget plot]
table {%
23 0.0401172637939453
23 0.0100553035736084
};
\addplot [black, forget plot]
table {%
23 0.13330078125
23 0.272943258285522
};
\addplot [black, forget plot]
table {%
22.875 0.0100553035736084
23.125 0.0100553035736084
};
\addplot [black, forget plot]
table {%
22.875 0.272943258285522
23.125 0.272943258285522
};
\addplot [line width=1pt, color5]
table {%
23.75 0.0278849601745605
24.25 0.0278849601745605
24.25 0.0477474512567307
24.125 0.0493659973144531
24.25 0.0509845433721755
24.25 0.0779881477355957
23.75 0.0779881477355957
23.75 0.0509845433721755
23.875 0.0493659973144531
23.75 0.0477474512567307
23.75 0.0278849601745605
};
%\addlegendentry{12.0 * 12.0}
\addplot [black, forget plot]
table {%
24 0.0278849601745605
24 0.010033130645752
};
\addplot [black, forget plot]
table {%
24 0.0779881477355957
24 0.149571895599365
};
\addplot [black, forget plot]
table {%
23.875 0.010033130645752
24.125 0.010033130645752
};
\addplot [black, forget plot]
table {%
23.875 0.149571895599365
24.125 0.149571895599365
};
\addplot [line width=1pt, color6]
table {%
24.75 0.0276931524276733
25.25 0.0276931524276733
25.25 0.0561063199907585
25.125 0.0584795475006104
25.25 0.0608527750104622
25.25 0.101002335548401
24.75 0.101002335548401
24.75 0.0608527750104622
24.875 0.0584795475006104
24.75 0.0561063199907585
24.75 0.0276931524276733
};
%\addlegendentry{16.0 * 16.0}
\addplot [black, forget plot]
table {%
25 0.0276931524276733
25 0.0100500583648682
};
\addplot [black, forget plot]
table {%
25 0.101002335548401
25 0.21076488494873
};
\addplot [black, forget plot]
table {%
24.875 0.0100500583648682
25.125 0.0100500583648682
};
\addplot [black, forget plot]
table {%
24.875 0.21076488494873
25.125 0.21076488494873
};
\addplot [color1, forget plot]
table {%
-0.125 0.133378744125366
0.125 0.133378744125366
};
\addplot [color1, forget plot]
table {%
0.875 0.0913627147674561
1.125 0.0913627147674561
};
\addplot [color1, forget plot]
table {%
1.875 0.0437288284301758
2.125 0.0437288284301758
};
\addplot [color1, forget plot]
table {%
2.875 0.196047306060791
3.125 0.196047306060791
};
\addplot [color1, forget plot]
table {%
3.875 0.0503287315368652
4.125 0.0503287315368652
};
\addplot [color1, forget plot]
table {%
4.875 0.0363602638244629
5.125 0.0363602638244629
};
\addplot [color1, forget plot]
table {%
9.875 0.217644453048706
10.125 0.217644453048706
};
\addplot [color1, forget plot]
table {%
10.875 0.124480247497559
11.125 0.124480247497559
};
\addplot [color1, forget plot]
table {%
11.875 0.0608000755310059
12.125 0.0608000755310059
};
\addplot [color1, forget plot]
table {%
12.875 0.0580892562866211
13.125 0.0580892562866211
};
\addplot [color1, forget plot]
table {%
13.875 0.0366926193237305
14.125 0.0366926193237305
};
\addplot [color1, forget plot]
table {%
14.875 0.053499698638916
15.125 0.053499698638916
};
\addplot [color1, forget plot]
table {%
19.875 0.263442993164062
20.125 0.263442993164062
};
\addplot [color1, forget plot]
table {%
20.875 0.21213698387146
21.125 0.21213698387146
};
\addplot [color1, forget plot]
table {%
21.875 0.11083984375
22.125 0.11083984375
};
\addplot [color1, forget plot]
table {%
22.875 0.0806457996368408
23.125 0.0806457996368408
};
\addplot [color1, forget plot]
table {%
23.875 0.0493659973144531
24.125 0.0493659973144531
};
\addplot [color1, forget plot]
table {%
24.875 0.0584795475006104
25.125 0.0584795475006104
};
\end{axis}

\end{tikzpicture}


==> tex/vio_uwb_gps_err.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color0}{rgb}{0.91796875,0.25,0.203125}
\definecolor{color1}{rgb}{0.6328125,0.203125,0.91796875}
\definecolor{color2}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color3}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color4}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
% \definecolor{color5}{rgb}{0.854901960784314,0.647058823529412,0.125490196078431}
% \definecolor{color6}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
% \definecolor{color7}{rgb}{0.627450980392157,0.32156862745098,0.176470588235294}

\definecolor{color7}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color6}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.91796875,0.25,0.203125}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    tick align=outside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    xtick style={color=black},
    y grid style={white!90!black},
    ymajorgrids,
    ytick style={color=black},
    scaled y ticks = false,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=0.666,
      text opacity=1,
      at={(0.97,0.97)},
      anchor=north east,
      draw=white!80!black
    },
    tick align=outside,
    tick pos=left,
    %
    %
    %
    %
    %
    %
    %
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
    % tick align=outside,
    % tick pos=left,
    % x grid style={white!69.0196078431373!black},
    xmin=0.5, xmax=7.5,
    % xtick style={color=black},
    xtick={1,2,3,4,5,6,7},
    xticklabels={$VIO_{xy}$, $UWB_{xy}$, $GPS_{xy}$, , $VIO_z$, $UWB_z$, $GPS_z$},
    % y grid style={white!69.0196078431373!black},
    ylabel={Error (m)},
    ymajorgrids,
    ymin=0.110018668126381, ymax=12.822998030654,
    ymode=log,
    % ytick style={color=black}
]
\addplot [line width=2pt, color0, forget plot]
table {%
0.75 0.438256200984864
1.25 0.438256200984864
1.25 0.674593597279193
1.125 0.698461927361191
1.25 0.722330257443189
1.25 0.940177507410002
0.75 0.940177507410002
0.75 0.722330257443189
0.875 0.698461927361191
0.75 0.674593597279193
0.75 0.438256200984864
};
% \addlegendentry{VIO}
\addplot [black, forget plot]
table {%
1 0.438256200984864
1 0.0632751893602295
};
\addplot [black, forget plot]
table {%
1 0.940177507410002
1 1.69229048091101
};
\addplot [black, forget plot]
table {%
0.875 0.0632751893602295
1.125 0.0632751893602295
};
\addplot [black, forget plot]
table {%
0.875 1.69229048091101
1.125 1.69229048091101
};
% \addlegendentry{UWB}
\addplot [line width=2pt, color2, forget plot]
table {%
1.75 0.623723617389486
2.25 0.623723617389486
2.25 0.939113143679274
2.125 0.981610969574021
2.25 1.02410879546877
2.25 1.50084906283514
1.75 1.50084906283514
1.75 1.02410879546877
1.875 0.981610969574021
1.75 0.939113143679274
1.75 0.623723617389486
};
\addplot [black, forget plot]
table {%
2 0.623723617389486
2 0.0267978777144759
};
\addplot [black, forget plot]
table {%
2 1.50084906283514
2 2.79929851920673
};
\addplot [black, forget plot]
table {%
1.875 0.0267978777144759
2.125 0.0267978777144759
};
\addplot [black, forget plot]
table {%
1.875 2.79929851920673
2.125 2.79929851920673
};
\addplot [line width=2pt, color3, forget plot]
table {%
2.75 1.60703157784121
3.25 1.60703157784121
3.25 2.55844096266862
3.125 2.6658632409173
3.25 2.77328551916597
3.25 3.8241523758089
2.75 3.8241523758089
2.75 2.77328551916597
2.875 2.6658632409173
2.75 2.55844096266862
2.75 1.60703157784121
};
\addplot [black, forget plot]
table {%
3 1.60703157784121
3 0.0147874407403017
};
\addplot [black, forget plot]
table {%
3 3.8241523758089
3 6.51091049405551
};
\addplot [black, forget plot]
table {%
2.875 0.0147874407403017
3.125 0.0147874407403017
};
\addplot [black, forget plot]
table {%
2.875 6.51091049405551
3.125 6.51091049405551
};
\addplot [line width=2pt, color4, forget plot]
table {%
3.75 nan
4.25 nan
4.25 nan
4.125 nan
4.25 nan
4.25 nan
3.75 nan
3.75 nan
3.875 nan
3.75 nan
3.75 nan
};
\addplot [black, forget plot]
table {%
4 nan
4 nan
};
\addplot [black, forget plot]
table {%
4 nan
4 nan
};
\addplot [black, forget plot]
table {%
3.875 nan
4.125 nan
};
\addplot [black, forget plot]
table {%
3.875 nan
4.125 nan
};
\addplot [line width=2pt, color5, forget plot]
table {%
4.75 0.2863183199475
5.25 0.2863183199475
5.25 0.366798369904502
5.125 0.47536206777
5.25 0.583925765635498
5.25 2.5692779101575
4.75 2.5692779101575
4.75 0.583925765635498
4.875 0.47536206777
4.75 0.366798369904502
4.75 0.2863183199475
};
\addplot [black, forget plot]
table {%
5 0.2863183199475
5 0.0066105721099996
};
\addplot [black, forget plot]
table {%
5 2.5692779101575
5 4.08462203046
};
\addplot [black, forget plot]
table {%
4.875 0.0066105721099996
5.125 0.0066105721099996
};
\addplot [black, forget plot]
table {%
4.875 4.08462203046
5.125 4.08462203046
};
\addplot [line width=2pt, color6, forget plot]
table {%
5.75 0.17235825
6.25 0.17235825
6.25 0.324021683390278
6.125 0.344904499999998
6.25 0.365787316609718
6.25 0.603364999999999
5.75 0.603364999999999
5.75 0.365787316609718
5.875 0.344904499999998
5.75 0.324021683390278
5.75 0.17235825
};
\addplot [black, forget plot]
table {%
6 0.17235825
6 0.000573000000000157
};
\addplot [black, forget plot]
table {%
6 0.603364999999999
6 1.249623
};
\addplot [black, forget plot]
table {%
5.875 0.000573000000000157
6.125 0.000573000000000157
};
\addplot [black, forget plot]
table {%
5.875 1.249623
6.125 1.249623
};
\addplot [line width=2pt, color7, forget plot]
table {%
6.75 1.68318462421337
7.25 1.68318462421337
7.25 2.84204411227774
7.125 3.0463188178633
7.25 3.25059352344885
7.25 5.89927187944771
6.75 5.89927187944771
6.75 3.25059352344885
6.875 3.0463188178633
6.75 2.84204411227774
6.75 1.68318462421337
};
\addplot [black, forget plot]
table {%
7 1.68318462421337
7 0.0253823215293938
};
\addplot [black, forget plot]
table {%
7 5.89927187944771
7 12.2124063625276
};
\addplot [black, forget plot]
table {%
6.875 0.0253823215293938
7.125 0.0253823215293938
};
\addplot [black, forget plot]
table {%
6.875 12.2124063625276
7.125 12.2124063625276
};
\addplot [color1, forget plot]
table {%
0.875 0.698461927361191
1.125 0.698461927361191
};
\addplot [color1, forget plot]
table {%
1.875 0.981610969574021
2.125 0.981610969574021
};
\addplot [color1, forget plot]
table {%
2.875 2.6658632409173
3.125 2.6658632409173
};
\addplot [color1, forget plot]
table {%
3.875 nan
4.125 nan
};
\addplot [color1, forget plot]
table {%
4.875 0.47536206777
5.125 0.47536206777
};
\addplot [color1, forget plot]
table {%
5.875 0.344904499999998
6.125 0.344904499999998
};
\addplot [color1, forget plot]
table {%
6.875 3.0463188178633
7.125 3.0463188178633
};
\end{axis}

\end{tikzpicture}


